Labelled calculi for the logics of rough concepts

We introduce sound and complete labelled sequent calculi for the basic normal non-distributive modal logic L and some of its axiomatic extensions, where the labels are atomic formulas of the first order language of enriched formal contexts, i.e., relational structures based on formal contexts which provide complete semantics for these logics. We also extend these calculi to provide a proof system for the logic of rough formal contexts.

==> calculus.tex <==

Below,  $p, q$ denote atomic propositions; $a, b, c$ (resp.~$x, y, z$) are labels corresponding to objects (resp.~features). Given labels $a$, $x$ and a modal formula $A$, well-formed formulas are of the type $a: A$ and $x:: A$, while $\varphi, \psi$ are meta-variables for well-formed formulas. Well-formed  terms are of any of the following shapes: $aIx$, $aR_\wbox x$, $x R_\wdia a$, $aR_\bbox x$, $x R_\bdia a$, and $t_1 \Rarr t_2$, where $t_1$ is of any of the following shapes:  $a R_\wbox x$, $a R_\bbox x$, $y R_\wdia a$, $y R_\bdia a$, $a R_\rhd b$, $a R_\blacktriangleright b$,  and $t_2$ is of the form $a I y$. Relational terms $t_1 \Rarr t_2$ are interpreted as $\forall u (t_1 \rightarrow t_2)$ where $u$ is the variable shared by $t_1$ and $t_2$. %$a$ if $t_1 = aR_\wbox x$ or $t_1 = a R_\bbox x$, and $u$ is $x$ if $t_1 = xR_\wdia a$ or $t_1 = x R_\bdia a$.
A sequent is an expression of the form $\Gamma \vd \Delta$, where $\Gamma, \Delta$ are meta-variables for multisets of well-formed formulas or terms. For any labels $u$, $v$ and relations $R$, $S$ we write $u (R;S) v$ as a shorthand for the term $w S v \Rarr u R w$. 

%Sequents $\Gamma \vd \Delta$ are interpreted as $\bigwedge \Gamma \implies \bigvee \Delta$. Well-formed formulas of the type $a: \varphi$ (resp.~$x:: \varphi$) are interpreted as $a \Vdash \varphi$ (resp.~$x \succ \varphi$).

\subsection{Labelled calculus for the basic $\mathcal{L}$-logic}
\label{sec:calculus}
{{\centering
\begin{tabular}{c}
\mc{1}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Initial rules and cut rules}\rule[-1.85mm]{0mm}{6mm}} \\
\AXC{$\ $}
\LL{Id$_{\,a:p}$}
\UIC{$\Gamma, a: p \vd a: p, \Delta$}
\DP
 \   
\AXC{$\ $}
\RL{Id$_{\,x::p}$}
\UIC{$\Gamma, x:: p \vd x:: p, \Delta$}
\DP
 \ \  
\AXC{$ \ $}
\LL{$\bot$}
\UIC{$\Gamma \vd x:: \bot, \Delta$}
\DP 
 \   
\AXC{$ \ $}
\RL{$\top$}
\UIC{$\Gamma \vd a: \top, \Delta$}
\DP
\\[\rulespace]
\AXC{$\Gamma \vd a: A, \Delta$}
\AXC{$\Gamma', a: A \vd \Delta'$}
\LL{Cut$_{\,aa}$}
\BIC{$\Gamma, \Gamma' \vd \Delta, \Delta'$}
\DP
 \  \ 
\AXC{$\Gamma \vd x:: A, \Delta$}
\AXC{$\Gamma', x:: A \vd \Delta'$}
\RL{Cut$_{\,xx}$}
\BIC{$\Gamma, \Gamma' \vd  \Delta, \Delta'$}
\DP \\[\rulespace]
%\AXC{$\Gamma \vd a: A, \Delta$}
%\AXC{$\Gamma'  \vd x:: A,  \Delta'$}
%\LL{Cut$_{\,ax}$}
%\BIC{$\Gamma, \Gamma' \vd a I x, \Delta, \Delta'$}
%\DP
\end{tabular}
\par}}
%\marginnote{AP: if we remove the heterogeneous cut in the other paper we should remove it here as well}

{{\centering
\begin{tabular}{rl}
\mc{2}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Switch rules$^\ast$} \rule[-1.85mm]{0mm}{6mm}}\\
\AXC{$\Gamma,  x:: B \vd x:: A, \Delta$}
\LL{S$xa$}
\UIC{$\Gamma,  a: A \vd  a: B, \Delta $}
\DP
 \ & \  
\AXC{$\Gamma,  a: A \vd  a: B, \Delta $}
\RL{S$ax$}
\UIC{$\Gamma,  x:: B \vd x:: A, \Delta$}
\DP
 \\[\rulespace]
\ \ \ \ 
\AXC{$ \Gamma, y R_\wdia a \Rarr b I y   \vd   b:A , \Delta $}
\LL{S$a \wdia x$}
\UIC{$\Gamma, x::A \vd x R_\Diamond a, \Delta$}
\DP
 \ & \ 
\AXC{$ \Gamma,a: A  \vd   a R_\wbox x, \Delta $}
\RL{S$ a \wbox x$}
\UIC{$\Gamma,  b R_\wbox x \Rarr b I y  \vd  y::A, \Delta$}
\DP
 \\[\rulespace]
\AXC{$\Gamma,  b R_\wbox x \Rarr b I y  \vd  y::A, \Delta$}
\LL{S$ x\wbox a$}
\UIC{$ \Gamma,a: A \vd   a R_\wbox x, \Delta $}
\DP
\ & \ 
\AXC{$\Gamma, x::A \vd x R_\Diamond a, \Delta$}
\RL{S$ x \wdia a$}
\UIC{$ \Gamma, y R_\wdia a \Rarr b I y   \vd   b:A , \Delta $}
\DP
 \\[\rulespace]
\AXC{$ \Gamma, b:A  \vd    y R_\wdia a \Rarr b I y , \Delta $}
\LL{S$ a \wdia x$}
\UIC{$\Gamma, x R_\Diamond a \vd  x::A, \Delta$}
\DP
 \ & \ 
\AXC{$ \Gamma,a: A  \vd   a R_\wbox x, \Delta $}
\RL{S$ a \wbox x $}
\UIC{$\Gamma, y:: A \vd b R_\wbox x \Rarr b I y, \Delta$}
\DP
 \\[\rulespace]
\AXC{$\Gamma,  y::A \vd   b R_\wbox x \Rarr b I y, \Delta$}
\LL{S$ x\wbox a $}
\UIC{$ \Gamma,a R_\wbox x\vd  a: A   , \Delta $}
\DP
\ & \ 
\AXC{$\Gamma, x R_\Diamond a \vd  x::A , \Delta$}
\RL{S$ x \wdia a $}
\UIC{$ \Gamma,b:A    \vd   y R_\wdia a \Rarr b I y,  \Delta $}
\DP
 \\[\rulespace]
\AXC{$\Gamma,     b R_\rhd a \Rarr b I y \vd y::A,  \Delta$}
\LL{S$ x{\rhd} a$}
\UIC{$ \Gamma,  c: A   \vd  c R_\rhd a, \Delta $}
\DP
\ & \ 
\AXC{$ \Gamma,c:A    \vd   c R_\rhd a,  \Delta $}
\RL{S$ a {\rhd} x $}
\UIC{$\Gamma,     b R_\rhd a \Rarr b I y \vd y::A,  \Delta$}
\DP
 \\[\rulespace]
 \AXC{$\Gamma,   y::A    \vd b R_\rhd a \Rarr b I y, \Delta$}
\LL{S$ x{\rhd} a$}
\UIC{$ \Gamma, c R_\rhd a   \vd   c: A , \Delta $}
\DP
\ & \ 
\AXC{$ \Gamma, c R_\rhd a \vd  c:A   ,  \Delta $}
\RL{S$ a {\rhd} x $}
\UIC{$\Gamma, y::A    \vd  b R_\rhd a \Rarr b I y,  \Delta$}
\DP
 \\[\rulespace]
\mc{2}{p{0.9\textwidth}}{\centering ${}^\ast$Side condition: the variables  $x,y,a,b$  occurring as labels of a formula in the premise of any of these rules must not occur in $\Gamma, \Delta$.}
\\
\end{tabular}
\par}}

Switch rules  for  $R_\bbox$,  $R_\bdia$, and $R_\blacktriangleright$ are analogous to those for $R_\wbox$,  $R_\wdia$, and $R_\rhd$. These rules encode the I-compatibility conditions of the relations $R_\bbox$,  $R_\bdia$,$R_\blacktriangleright$,$R_\wbox$,  $R_\wdia$, and $R_\rhd$ as demonstrated by their soundness proof shown in Section \ref{ssec:soundness}.

{{\centering
\begin{tabular}{rl}
\mc{2}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Approximation rules$^*$} \rule[-1.85mm]{0mm}{6mm}}\\
 \AXC{$\Gamma,  x:: A \vd aIx, \Delta$}
\LL{$approx_x$}
\UIC{$ \Gamma \vd a: A, \Delta $}
\DP
\ & \ 
  \AXC{$\Gamma,  a: A \vd aIx, \Delta$}
\RL{$approx_a$}
\UIC{$ \Gamma \vd   x::A, \Delta $}
\DP
 \\[\rulespace]
\mc{2}{p{0.9\textwidth}}{\centering${}^\ast$Side condition: the variables  $x,y$  occurring as labels of a formula in the premise of any of these rules must not occur in $\Gamma, \Delta$.}
\\
\end{tabular}
\par}}

\noindent For  $T, T'\in \{R_\wdia,\, J,\, J;I,\, J;R_\wbox,\, J;R_\rhd,\, R_\bdia,\, J;R_\bbox,\, J;R_\blacktriangleright \}$ and  $S, S'\in \{R_\wbox,\, I,\, I;J,\, I;R_\wdia,\, I;R_\bdia, \, R_\bbox\}$ and for all labels  $u,v, w$ of the form $a$ or $x$, we have the following switch rules:

{{\centering
\begin{tabular}{rl}
\mc{2}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Pure structure switch rules$^*$} \rule[-1.85mm]{0mm}{6mm}}\\
 \AXC{$\Gamma,  x T u    \vd x T' v, \Delta$}
\LL{S$(I;S)$}
\UIC{$ \Gamma, a (I;T') v  \vd   a (I;T) u, \Delta $}
\DP
\ & \ 
  \AXC{$\Gamma,  a S u    \vd a S' v, \Delta$}
\RL{-S$(J;T)$}
\UIC{$ \Gamma, x (J;S') v  \vd   x (J;S) u, \Delta $}
\DP
 \\[\rulespace]
 \AXC{$ \Gamma, a (I;T') v  \vd   a (I;T) u, \Delta $}
\LL{-S$(I;S)$}
\UIC{$\Gamma,  x T u    \vd x T' v, \Delta$}
\DP
\ & \ 
  \AXC{$ \Gamma, x (J;S') v  \vd   x (J;S) u, \Delta $}
\RL{S$-(J;T)$}
\UIC{$\Gamma,  a S u    \vd a S' v, \Delta$}
\DP
 \\[\rulespace]
 \AXC{$\Gamma   \vd  a S u, \Delta$}
\LL{Id$(I;J)_R$}
\UIC{$ \Gamma    \vd   a (I;(J;S)) u , \Delta $}
\DP
\ & \ 
\AXC{$\Gamma   \vd  x T u, \Delta$}
\RL{Id$(J;I)_R$}
\UIC{$ \Gamma    \vd   x (J;(I;T)) u , \Delta $}
\DP
 \\[\rulespace]
 \AXC{$\Gamma,  a S u \vd  \Delta$}
\LL{Id$(I;J)_L$}
\UIC{$ \Gamma, a (I;(J;S)) u    \vd    \Delta $}
\DP
\ & \ 
\AXC{$\Gamma,  x T u  \vd  \Delta$}
\RL{Id$(J;I)_L$}
\UIC{$ \Gamma, x (J;(I;T)) u     \vd   \Delta $}
\DP
 \\[\rulespace]
\mc{2}{p{0.9\textwidth}}{\centering${}^\ast$Side condition: the variable  $x$  (resp.~$a$) occurring  in the premise of  rules S$(I;S)$, -S$(I;S)$ (resp.~S$(J;T)$, -S$(J;T)$ ) must not occur in $\Gamma, \Delta$.}
\\
\end{tabular}
\par}}
The rules above  encode the definition of  $I$-composition of relations on formal contexts \cite[Definition3.10]{conradie2021rough}.

{{\centering
\begin{tabular}{rl}
\mc{2}{c}{\rule[-1.85mm]{0mm}{8mm} \textbf{Adjunction rules}\rule[-1.85mm]{0mm}{8mm}} \\

\AXC{$\Gamma \vd  x R_\wdia a,  \Delta$}
\LL{\fns $\wdia \dashv \bbox$}
\UIC{$\Gamma \vd a  R_\bbox x,  \Delta$}
\DP 
 \ & \  
\AXC{$\Gamma \vd a  R_\bbox x,  \Delta$}
\RL{\fns $\wdia \dashv \bbox^{-1}$}
\UIC{$\Gamma \vd x R_\wdia a,  \Delta$}
\DP
 \\[\rulespace]
 
\AXC{$\Gamma \vd a R_\wbox x,  \Delta$}
\LL{\fns $\bdia \dashv \wbox$}
\UIC{$\Gamma \vd  x R_\bdia a,  \Delta$}
\DP 
 \ & \  
\AXC{$\Gamma \vd x R_\bdia a,  \Delta$}
\RL{\fns $\bdia \dashv \wbox^{-1}$}
\UIC{$\Gamma \vd a R_\wbox x,  \Delta$}
\DP
 \\[\rulespace]
 
\AXC{$\Gamma \vd a R_\rhd b,  \Delta$}
\LL{\fns $\rhd \dashv \;\blacktriangleright$}
\UIC{$\Gamma \vd  b R_\blacktriangleright a,  \Delta$}
\DP 
 \ & \  
\AXC{$\Gamma \vd a R_\blacktriangleright b,  \Delta$}
\RL{\fns $\blacktriangleright \,\dashv \,\rhd$}
\UIC{$\Gamma \vd  b R_\rhd a,  \Delta$}
\DP 
\end{tabular}
\par}}
Adjunction rules  encode the fact that operators $\wdia$ and $\bbox$,  $\bdia$ and $\wbox$, and $\rhd$ and $\blacktriangleright$ constitute pairs of adjunction operators.  \marginnote{Fix alignment}
{{\centering
\begin{tabular}{rl}
\mc{2}{c}{\rule[-1.85mm]{0mm}{8mm} \textbf{Invertible logical rules for propositional connectives}\rule[-1.85mm]{0mm}{8mm}} \\

\AXC{$\Gamma, a : A, a: B \vd \Delta$}
\LL{$ \wedge_L$}
\UIC{$\Gamma, a : A \wedge B \vd \Delta$}
\DP
 \ & \  
\AXC{$\Gamma \vd a: A, \Delta$}
\AXC{$\Gamma \vd a: B, \Delta$}
\RL{$\wedge_R$}
\BIC{$\Gamma \vd a: A \wedge B, \Delta$}
\DP
 \\[\rulespace]

\AXC{$\Gamma \vd  x:: A, \Delta$}
\AXC{$\Gamma \vd  x:: B, \Delta$}
\LL{$\vee_L$}
\BIC{$\Gamma \vd  x:: A \vee B, \Delta$}
\DP
 \ & \  
\AXC{$\Gamma, x:: A, x:: B \vd \Delta$}
\RL{$ \vee_R$}
\UIC{$\Gamma, x:: A \vee B \vd \Delta$}
\DP

% & \\

%% & \\
%\AXC{$\Gamma \vd \nx : A, \Delta$}
%\LL{$\neg_L$}
%\UIC{$\Gamma, \nx : \neg A \vd \Delta$}
%\DP
%
% & 
%\AXC{$\Gamma, \nx : A \vd \Delta$}
%\RL{$\neg_R$}
%\UIC{$\Gamma \vd \nx : \neg A, \Delta$}
%\DP
% \\

% & \\

%\AXC{$\Gamma, A \Rarr B \vd A, \Delta$}
%\AXC{$\Gamma, B \vd \Delta$}
%\LL{$\Rarr_L$}
%\BIC{$\Gamma, A \Rarr B \vd A, \Delta$}
%\DP
% \ & \ 
%\AXC{$\Gamma, A \vd B, \Delta$}
%\RL{$\Rarr_R$}
%\UIC{$\Gamma \vd A \Rarr B, \Delta$}
%\DP
% \\
\end{tabular}
\par}}

{{\centering
\begin{tabular}{rl}

\mc{2}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Invertible logical rules for modal connectives${}^\ast$}\rule[-1.85mm]{0mm}{8mm}} \\

\AXC{$ \Gamma, a:\Box A  \vd x:: A, a R_\Box x, \Delta $}
\LL{$\wbox_L$}
\UIC{$\Gamma, a:\Box A \vd a R_\Box x, \Delta$}
\DP
 \ & \  
\AXC{$ \Gamma, x:: A \vd a R_\Box x, \Delta $}
\RL{$\Box_R$}
\UIC{$\Gamma \vd a: \Box A, \Delta$}
\DP
 \\[\rulespace]

\AXC{$\Gamma, a:A \vd x R_\Diamond a, \Delta $}
\LL{$\Diamond_L$}
\UIC{$\Gamma \vd x:: \Diamond A, \Delta$}
\DP
 \ & \   
%\AXC{$\Gamma,x R_\Diamond a,  a:A \implies x R_\Diamond a, x::\Diamond A  \vd  \Delta $}
%\RL{$R_\Diamond$???}
%\UIC{$\Gamma,  x:: \Diamond A  \vd x R_\Diamond a, \Delta$}
%\DP
\AXC{$\Gamma, x:: \Diamond A \vd  a:A, x R_\Diamond a, \Delta$}
\RL{$\Diamond_R$}
\UIC{$\Gamma,  x:: \Diamond A  \vd x R_\Diamond a, \Delta$}
\DP
 \\[\rulespace]
\AXC{$ \Gamma, a:\rhd A  \vd b: A, a R_\rhd b, \Delta $}
\LL{$\rhd_L$}
\UIC{$\Gamma, a:\rhd A \vd a R_\rhd b, \Delta$}
\DP
 \ & \  
\AXC{$ \Gamma, b: A \vd a R_\rhd b, \Delta $}
\RL{$\rhd_R$}
\UIC{$\Gamma \vd a: \rhd A, \Delta$}
\DP
 \\[\rulespace]
\mc{2}{p{0.8\textwidth}}{\centering${}^\ast$Side condition: the variable $x$ (resp.~$a$, resp.~$b$) must not occur in the conclusion of $\wbox_R$  (resp.~ $\wdia_L$, resp.~$\rhd_R$).} \\
\end{tabular}
\par}}
Logical rules encode the definition of satisfaction and refutation for propositional and modal connectives discussed in Section \ref{ssec:relsem}. 
\subsection{Relational calculi for the axiomatic extensions of the basic $\mathcal{L}$-logic } \label{ssec: Relational calculus extension}
The structural rule corresponding to each axiom listed in Table \ref{axiom table} is generated as the read-off of the first-order condition corresponding to the given axiom as listed in Proposition \ref{lemma:correspondences}. For any nonempty subset $\Sigma$ of modal axioms as reported in Table \ref{axiom table}, we let $G3N_P\Sigma$ denote the extension of $G3N_P$ with the corresponding rules.
%These are collected in the following table:
{\footnotesize{
\begin{table}
    \centering
   \begin{tabular}{|c|Sc||c|Sc|}
\hline
   \textbf{\quad  Modal axiom\quad } & \textbf{\quad \quad  Relational calculus rule \quad \quad  }&\textbf{\quad  Modal axiom\quad } & \textbf{\quad \quad  Relational calculus rule \quad \quad  }\\ 
   \hline
     $\wbox p \vd p$  &  \AXC{$\Gamma \vd a R_\wbox x, \Delta$}\UIC{$\Gamma \vd a I x, \Delta$} \DP %\\[2ex]
    %\hline
   &   $ p \vd \wdia p $ &  \AXC{$\Gamma \vd x R_\wdia a, \Delta$}\UIC{$\Gamma \vd a I x, \Delta$} \DP \\[2ex]
     \hline 
    $p \vd \wbox\wdia p$ &  \AXC{$\Gamma \vd x R_\wdia a, \Delta$}\UIC{$\Gamma \vd x R_\bdia a, \Delta$} \DP %\\[2ex]
   % \hline
     & $ \wdia \wbox p \vd  p $ &  \AXC{$\Gamma \vd x R_\bdia a, \Delta$}\UIC{$\Gamma \vd x R_\wdia a, \Delta$} \DP \\[2ex]
     \hline
      $\wbox p \vd \wbox\wbox p$ &  \AXC{$\Gamma  \vd  a R_\wbox x, \Delta$}\UIC{$\Gamma, b R_\wbox x \Rarr  y J b  \vd a R_\wbox y, \Delta$} \DP %\\[2ex]
      %\hline
    &  $ \wdia p \vd \wdia\wdia p $ &  \AXC{$\Gamma \vd x R_\wdia a, \Delta$}\UIC{$\Gamma, y R_\wdia a \Rarr b I y \vd  x R_\wdia b,  \Delta$} \DP \\[2ex]
     \hline 
      $  p \vd {\rhd}{\rhd} p $ &  \AXC{$\Gamma \vd a R_\rhd b, \Delta$}\UIC{$\Gamma \vd  b R_\rhd a,  \Delta$} \DP &&\\[2ex]
     \hline 
\end{tabular}
\vspace{0.2 cm}
    \caption{Modal axioms and their corresponding rules.}
    \label{axiom table}
\end{table}
}}
\subsection{The relational calculus $RG3N_P$ for the $\mathcal{L}$-logic of rough formal contexts}
\label{ssec: relational Kent calculus}

The calculus $G3N_P$ introduced in Section \ref{sec:calculus} can be specialized so as to capture the semantic environment of rough formal contexts by associating the connective $\kbox$ (resp.\ $\kdia$) with relational labels in which $\kentsbox$ (resp.\ $\kentsdiamond$) occurs, and adding rules encoding the reflexivity and the transitivity of $E$, rather than  the (equivalent, cf.~Lemma \ref{thm:equivalent_s_rewriting}) first-order conditions on  $\kentsbox$. We need the following set of switching rules encoding the relation between $E$ and $I$, and the $I$-compatibility of $E$ and $\kentsbox$ (and $\kentsdiamond$).
\smallskip

{{\centering
\begin{tabular}{rl}
 \mc{2}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Interdefinability rules}\rule[-1.85mm]{0mm}{6mm}} \\
\AXC{$\Gamma, b \kentsbox x \Rightarrow b I y \vd y :: A, \Delta$}
\LL{swSf$^*$}
\UIC{$\Gamma, a : A \vd a \kentsbox x, \Delta$}
\DP
 \quad\quad &
\AXC{$\Gamma, a : A \vd a \kentsbox x, \Delta$}
\RL{swSfi$^*$}
\UIC{$\Gamma, b \kentsbox x \Rightarrow b I y \vd y :: A, \Delta$}
\DP \\[\rulespace]

\AXC{$\Gamma, x :: A \vd x \kentsdiamond a, \Delta$}
\LL{swSdf$^*$}
\UIC{$\Gamma, b E a \vd b : A, \Delta$}
\DP
\quad\quad
&
\AXC{$\Gamma, b E a \vd b : A, \Delta$}
\RL{swSdfi$^*$}
\UIC{$\Gamma, x :: A \vd x \kentsdiamond a, \Delta$}
\DP \\[\rulespace]

\AXC{$\Gamma, a E c \vd a \kentsbox x, \Delta$}
\LL{swES$^*$}
\UIC{$\Gamma, b \kentsbox x \Rightarrow b I y \vd y \kentsdiamond a, \Delta$}
\DP \quad\quad
&
\AXC{$\Gamma, b \kentsbox x \Rightarrow b I y \vd y \kentsdiamond a, \Delta$}
\RL{swESi$^*$}
\UIC{$\Gamma, a E c \vd a \kentsbox x, \Delta$}
\DP\\[\rulespace]

\AXC{$\Gamma \vd a \kentsbox x, \Delta$}
\LL{curryS $^{**}$}
\UIC{$\Gamma, b E a \vd b I x, \Delta$}
\DP \quad\quad
&
\AXC{$\Gamma, b E a \vd b I x, \Delta$}
\RL{uncurryS $^{**}$}
\UIC{$\Gamma, \vd a \kentsbox x, \Delta$}
\DP \\
[\rulespace]
\mc{2}{p{0.8\textwidth}}{\centering \small ${}^\ast$Side condition: the variables  $y,a,b$  occurring as  labels to a formula in the premise of any of these rules do not occur in $\Gamma, \Delta$.} \\
\mc{2}{p{0.8\textwidth}}{\centering \small $^{\ast\ast}$Side condition: $b$ does not occur in $\Gamma$ nor in $\Delta$.} \\
\end{tabular}

\begin{tabular}{rcl}
 \mc{3}{c}{\rule[-1.85mm]{0mm}{8mm}\textbf{Rules for equivalence relations}\rule[-1.85mm]{0mm}{6mm}} \\
\AXC{$\Gamma,   a E a \vd  \Delta$}
\LL{refl}
\UIC{$\Gamma  \vd  \Delta$}
\DP \quad
&
\AXC{$\Gamma  \vd a E b, \Delta$}
\RL{sym}
\UIC{$\Gamma \vd b E a, \Delta$}
\DP \quad 
&
\AXC{$\Gamma  \vd a E b, b E c  \Delta$}
\RL{trans}
\UIC{$\Gamma  \vd  a E c, \Delta$}
\DP\\
\end{tabular}
\par}}
